Does Weak-to-strong Generalization Happen under Spurious Correlations?

We initiate a unified theoretical and algorithmic study of a key problem in weak-to-strong (W2S) generalization: when fine-tuning a strong pre-trained student with pseudolabels from a weaker teacher on a downstream task with spurious correlations, does W2S happen, and how to improve it upon failures? We consider two sources of spurious correlations caused by group imbalance: (i) a weak teacher fine-tuned on group-imbalanced labeled data with a minority group of fraction $\eta_\ell$, and (ii) a group-imbalanced unlabeled set pseudolabeled by the teacher with a minority group of fraction $\eta_u$. Theoretically, a precise characterization of W2S gain at the proportional asymptotic limit shows that W2S always happens with sufficient pseudolabels when $\eta_u = \eta_\ell$ but may fail when $\eta_u \ne \eta_\ell$, where W2S gain diminishes as $(\eta_u - \eta_\ell)^2$ increases. Our theory is corroborated by extensive experiments on various spurious correlation benchmarks and teacher-student pairs. To boost W2S performance upon failures, we further propose a simple, effective algorithmic remedy that retrains the strong student on its high-confidence data subset after W2S fine-tuning. Our algorithm is group-label-free and achieves consistent, substantial improvements over vanilla W2S fine-tuning.

==> utils.tex <==
\RequirePackage{algorithm,algpseudocode}
\RequirePackage{amsmath,amsfonts,amsthm,amssymb}
\RequirePackage{xcolor,xspace,tcolorbox}

\definecolor{mdarkred}{HTML}{7b241c}
\definecolor{mdarkgreen}{HTML}{0b5345}
\definecolor{mdarkblue}{HTML}{000066} 
\definecolor{morange}{HTML}{f57c00}
\definecolor{mgreen}{HTML}{388e3c}
\definecolor{mviolet}{HTML}{7b1fa2}
\definecolor{mlightyellow}{HTML}{fbeee6}
\definecolor{mlightred}{HTML}{f2d7d5} 
\definecolor{mlightgreen}{HTML}{d4efdf}
\definecolor{mlightblue}{HTML}{d6eaf8}
\definecolor{mlightviolet}{HTML}{ebdef0}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\gray}[1]{\textcolor{gray}{#1}}
\newcommand{\orange}[1]{\textcolor{morange}{#1}}
\newcommand{\green}[1]{\textcolor{mgreen}{#1}}
\newcommand{\violet}[1]{\textcolor{mviolet}{#1}}

% \hypersetup{
%     pdftoolbar=true,        % show Acrobat’s toolbar?
%     pdfmenubar=true,        % show Acrobat’s menu?
%     pdffitwindow=false,     % window fit to page when opened
%     pdfnewwindow=true,      % links in new window
%     colorlinks=true,
%     linkcolor=mdarkblue,
%     citecolor=mdarkblue,
%     filecolor=mdarkblue,
%     urlcolor=mdarkblue,
% }
% pagebackref 
% \renewcommand*{\backrefalt}[4]{%
% \ifcase #1 %
% (Not cited.)%
% \or
% (Cited on page #2.)%
% \else
% (Cited on pages #2.)%
% \fi
% }

% If you defined \newtheorem{assumption}{Assumption}, then add:
\crefname{assumption}{assumption}{assumptions}
\Crefname{assumption}{Assumption}{Assumptions}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{return}}

% footnote
\let\svthefootnote\thefootnote
\newcommand\freefootnote[1]{%
  \let\thefootnote\relax%
  \footnotetext{#1}%
  \let\thefootnote\svthefootnote%
}

\makeatletter
\newcommand\footnoteref[1]{\protected@xdef\@thefnmark{\ref{#1}}\@footnotemark}
\makeatother

% colorbox
\newtcolorbox{tbox}[3][]{%
    colframe=#2!50,colback=#2!10,coltitle=#2!20!black,title={\color{white}#3},#1
}
\newtcolorbox{redtbox}[2][]{%
    colframe=mdarkred!50,colback=mdarkred!10,coltitle=mdarkred!20!black,title={\color{white}#2},#1
}
\newtcolorbox{greentbox}[2][]{%
    colframe=mdarkgreen!50,colback=mdarkgreen!10,coltitle=mdarkgreen!20!black,title={\color{white}#2},#1
}
\newtcolorbox{bluetbox}[2][]{%
    colframe=mdarkblue!50,colback=mdarkblue!10,coltitle=mdarkblue!20!black,title={\color{white}#2},#1
}
\newtcolorbox{violettbox}[2][]{%
    colframe=mviolet!50,colback=mviolet!10,coltitle=mviolet!20!black,title={\color{white}#2},#1
}
\newtcolorbox{yellowtbox}[2][]{%
    colframe=morange!50,colback=morange!10,coltitle=morange!20!black,title={\color{white}#2},#1
}

%%%%%%%%%%%%%%% Special characters %%%%%%%%%%%%%%%
\newcommand{\A}{\mathbb{A}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\C}{\mathbb{C}} % complex field
\newcommand{\D}{\mathbb{D}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\JJ}{\mathbb{J}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\N}{\mathbb{N}} % nature numbers
\newcommand{\OO}{\mathbb{O}} % nature numbers
\newcommand{\PP}{\mathbb{P}} % nature numbers
\newcommand{\Q}{\mathbb{Q}} % rational field 
\newcommand{\R}{\mathbb{R}} % real field
\newcommand{\SSS}{\mathbb{S}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\U}{\mathbb{U}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\W}{\mathbb{W}}
\newcommand{\X}{\mathbb{X}}
\newcommand{\Y}{\mathbb{Y}}
\newcommand{\Z}{\mathbb{Z}} % integer field



% bold
\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\renewcommand{\sb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}


\newcommand{\abd}{\boldsymbol{a}}
\newcommand{\bbd}{\boldsymbol{b}}
\newcommand{\cbd}{\boldsymbol{c}}
\newcommand{\dbd}{\boldsymbol{d}}
\newcommand{\ebd}{\boldsymbol{e}}
\newcommand{\fbd}{\boldsymbol{f}}
\newcommand{\gbd}{\boldsymbol{g}}
\newcommand{\hbd}{\boldsymbol{h}}
\newcommand{\ibd}{\boldsymbol{i}}
\newcommand{\jbd}{\boldsymbol{j}}
\newcommand{\kbd}{\boldsymbol{k}}
\newcommand{\lbd}{\boldsymbol{l}}
\newcommand{\mbd}{\boldsymbol{m}}
\newcommand{\nbd}{\boldsymbol{n}}
\newcommand{\obd}{\boldsymbol{o}}
\newcommand{\pbd}{\boldsymbol{p}}
\newcommand{\qbd}{\boldsymbol{q}}
\newcommand{\rbd}{\boldsymbol{r}}
\newcommand{\sbd}{\boldsymbol{s}}
\newcommand{\tbd}{\boldsymbol{t}}
\newcommand{\ubd}{\boldsymbol{u}}
\newcommand{\vbd}{\boldsymbol{v}}
\newcommand{\wbd}{\boldsymbol{w}}
\newcommand{\xbd}{\boldsymbol{x}}
\newcommand{\ybd}{\boldsymbol{y}}
\newcommand{\zbd}{\boldsymbol{z}}

\newcommand{\Abd}{\boldsymbol{A}}
\newcommand{\Bbd}{\boldsymbol{B}}
\newcommand{\Cbd}{\boldsymbol{C}}
\newcommand{\Dbd}{\boldsymbol{D}}
\newcommand{\Ebd}{\boldsymbol{E}}
\newcommand{\Fbd}{\boldsymbol{F}}
\newcommand{\Gbd}{\boldsymbol{G}}
\newcommand{\Hbd}{\boldsymbol{H}}
\newcommand{\Ibd}{\boldsymbol{I}}
\newcommand{\Jbd}{\boldsymbol{J}}
\newcommand{\Kbd}{\boldsymbol{K}}
\newcommand{\Lbd}{\boldsymbol{L}}
\newcommand{\Mbd}{\boldsymbol{M}}
\newcommand{\Nbd}{\boldsymbol{N}}
\newcommand{\Obd}{\boldsymbol{O}}
\newcommand{\Pbd}{\boldsymbol{P}}
\newcommand{\Qbd}{\boldsymbol{Q}}
\newcommand{\Rbd}{\boldsymbol{R}}
\newcommand{\Sbd}{\boldsymbol{S}}
\newcommand{\Tbd}{\boldsymbol{T}}
\newcommand{\Ubd}{\boldsymbol{U}}
\newcommand{\Vbd}{\boldsymbol{V}}
\newcommand{\Wbd}{\boldsymbol{W}}
\newcommand{\Xbd}{\boldsymbol{X}}
\newcommand{\Ybd}{\boldsymbol{Y}}
\newcommand{\Zbd}{\boldsymbol{Z}}


\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\Afrak}{\mathfrak{A}}
\newcommand{\Bfrak}{\mathfrak{B}}
\newcommand{\Cfrak}{\mathfrak{C}}
\newcommand{\Dfrak}{\mathfrak{D}}
\newcommand{\Efrak}{\mathfrak{E}}
\newcommand{\Ffrak}{\mathfrak{F}}
\newcommand{\Gfrak}{\mathfrak{G}}
\newcommand{\Hfrak}{\mathfrak{H}}
\newcommand{\Ifrak}{\mathfrak{I}}
\newcommand{\Jfrak}{\mathfrak{J}}
\newcommand{\Kfrak}{\mathfrak{K}}
\newcommand{\Lfrak}{\mathfrak{L}}
\newcommand{\Mfrak}{\mathfrak{M}}
\newcommand{\Nfrak}{\mathfrak{N}}
\newcommand{\Ofrak}{\mathfrak{O}}
\newcommand{\Pfrak}{\mathfrak{P}}
\newcommand{\Qfrak}{\mathfrak{Q}}
\newcommand{\Rfrak}{\mathfrak{R}}
\newcommand{\Sfrak}{\mathfrak{S}}
\newcommand{\Tfrak}{\mathfrak{T}}
\newcommand{\Ufrak}{\mathfrak{U}}
\newcommand{\Vfrak}{\mathfrak{V}}
\newcommand{\Wfrak}{\mathfrak{W}}
\newcommand{\Xfrak}{\mathfrak{X}}
\newcommand{\Yfrak}{\mathfrak{Y}}
\newcommand{\Zfrak}{\mathfrak{Z}}

\newcommand{\afrak}{\mathfrak{a}}
\newcommand{\bfrak}{\mathfrak{b}}
\newcommand{\cfrak}{\mathfrak{c}}
\newcommand{\dfrak}{\mathfrak{d}}
\newcommand{\efrak}{\mathfrak{e}}
\newcommand{\ffrak}{\mathfrak{f}}
\newcommand{\gfrak}{\mathfrak{g}}
\newcommand{\hfrak}{\mathfrak{h}}
\newcommand{\ifrak}{\mathfrak{i}}
\newcommand{\jfrak}{\mathfrak{j}}
\newcommand{\kfrak}{\mathfrak{k}}
\newcommand{\lfrak}{\mathfrak{l}}
\newcommand{\mfrak}{\mathfrak{m}}
\newcommand{\nfrak}{\mathfrak{n}}
\newcommand{\ofrak}{\mathfrak{o}}
\newcommand{\pfrak}{\mathfrak{p}}
\newcommand{\qfrak}{\mathfrak{q}}
\newcommand{\rfrak}{\mathfrak{r}}
\newcommand{\sfrak}{\mathfrak{s}}
\newcommand{\tfrak}{\mathfrak{t}}
\newcommand{\ufrak}{\mathfrak{u}}
\newcommand{\vfrak}{\mathfrak{v}}
\newcommand{\wfrak}{\mathfrak{w}}
\newcommand{\xfrak}{\mathfrak{x}}
\newcommand{\yfrak}{\mathfrak{y}}
\newcommand{\zfrak}{\mathfrak{z}}

% Greek
\newcommand{\eps}{\epsilon}
\newcommand{\veps}{\varepsilon}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\deltab}{\boldsymbol{\delta}}
\newcommand{\epsb}{\boldsymbol{\eps}}
\newcommand{\vepsb}{\boldsymbol{\veps}}
\newcommand{\zetab}{\boldsymbol{\zeta}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\vthetab}{\boldsymbol{\vartheta}}
\newcommand{\iotab}{\boldsymbol{\iota}}
\newcommand{\kappab}{\boldsymbol{\kappa}}
\newcommand{\vkappab}{\boldsymbol{\varkappa}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\nub}{\boldsymbol{\nu}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\omicronb}{\boldsymbol{\omicron}}
\newcommand{\pib}{\boldsymbol{\pi}}
\newcommand{\vpib}{\boldsymbol{\varpi}}
\newcommand{\rhob}{\boldsymbol{\rho}}
\newcommand{\vrhob}{\boldsymbol{\varrho}}
\newcommand{\sigmab}{\boldsymbol{\sigma}}
\newcommand{\vsigmab}{\boldsymbol{\varsigma}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\upsilonb}{\boldsymbol{\upsilon}}
\newcommand{\phib}{\boldsymbol{\phi}}
\newcommand{\vphib}{\boldsymbol{\varphi}}
\newcommand{\chib}{\boldsymbol{\chi}}
\newcommand{\psib}{\boldsymbol{\psi}}
\newcommand{\omegab}{\boldsymbol{\omega}}
\newcommand{\varepsb}{\boldsymbol{\varepsilon}}

\newcommand{\Alphab}{\boldsymbol{\Alpha}}
\newcommand{\Betab}{\boldsymbol{\Beta}}
\newcommand{\Gammab}{\boldsymbol{\Gamma}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\Epsb}{\boldsymbol{\Epsilon}}
\newcommand{\Zetab}{\boldsymbol{\Zeta}}
\newcommand{\Etab}{\boldsymbol{\Eta}}
\newcommand{\Thetab}{\boldsymbol{\Theta}}
\newcommand{\Iotab}{\boldsymbol{\Iota}}
\newcommand{\Kappab}{\boldsymbol{\Kappa}}
\newcommand{\Lambdab}{\boldsymbol{\Lambda}}
\newcommand{\Mub}{\boldsymbol{\Mu}}
\newcommand{\Nub}{\boldsymbol{\Nu}}
\newcommand{\Xib}{\boldsymbol{\Xi}}
\newcommand{\Omicronb}{\boldsymbol{\Omicron}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\Rhob}{\boldsymbol{\Rho}}
\newcommand{\Sigmab}{\boldsymbol{\Sigma}}
\newcommand{\Taub}{\boldsymbol{\Tau}}
\newcommand{\Upsilonb}{\boldsymbol{\Upsilon}}
\newcommand{\Phib}{\boldsymbol{\Phi}}
\newcommand{\Chib}{\boldsymbol{\Chi}}
\newcommand{\Psib}{\boldsymbol{\Psi}}
\newcommand{\Omegab}{\boldsymbol{\Omega}}








%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%
\renewcommand{\le}{\leqslant}
\renewcommand{\ge}{\geqslant}
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\newcommand{\dfeq}{\triangleq}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}
\newcommand{\pinv}{\dagger}
\newcommand*{\poly}{\mathop{\mathrm{poly}}}
\newcommand*{\mean}{\mathop{\mathrm{mean}}}
\newcommand*{\median}{\mathop{\mathrm{median}}}
\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\range}{\mathop{\mathrm{Range}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\prox}{\mathop{\mathrm{prox}}}
\newcommand{\proj}{\mathop{\mathrm{proj}}}
\newcommand{\spn}{\mathop{\mathrm{span}}}
\newcommand{\row}{\mathop{\mathrm{row}}}
\newcommand{\col}{\mathop{\mathrm{col}}}
\newcommand{\nucnorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}
\newcommand{\pto}{\mathrel{\ooalign{\hfil$\mapstochar\mkern5mu$\hfil\cr$\to$\cr}}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}

\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{\partial #1^2}}
\newcommand{\pnwrt}[2]{\frac{\partial^#1}{\partial #2^#1}}
\newcommand{\pfrac}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\ppfrac}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\pnfrac}[3]{\frac{\partial^#1 #2}{\partial #3^#1}}

\newcommand{\rademacher}{\mathop{\mathrm{Rad}}}
\newcommand{\unif}{\mathop{\mathrm{Unif}}}
\newcommand{\exrisk}{\mathbf{ER}}
\newcommand{\loc}[2]{\sbr{#1}_{#2}}
\newcommand{\tsvd}[2]{\ssbr{#1}_{#2}}
\newcommand{\sval}[2]{\sigma_{#2}(#1)}



%%%%%%%%%%%%%%% Super/sup-scripts %%%%%%%%%%%%%%%
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\ol}[1]{\overline{#1}} % overline
\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}




%%%%%%%%%%%%%%% Short Forms %%%%%%%%%%%%%%%
\newcommand{\ea}{\emph{et al.}\xspace}
\newcommand{\eg}{\emph{e.g.}\xspace}
\newcommand{\ie}{\emph{i.e.}\xspace}
\newcommand{\iid}{\emph{i.i.d.}\xspace}
\newcommand{\cf}{\emph{cf.}\xspace}
\newcommand{\wrt}{\emph{w.r.t.}\xspace}
\newcommand{\st}{\emph{s.t.}\xspace}
\newcommand{\whp}{\emph{w.h.p.}\xspace}



%%%%%%%%%%%%%%% Brackets %%%%%%%%%%%%%%
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abbr}[1]{\left\vert#1\right\vert}
\newcommand{\abr}[1]{\langle#1\rangle}
% \newcommand{\ssbr}[1]{[\![ #1 ]\!]}
\newcommand{\ssbr}[1]{\left\llbracket #1 \right\rrbracket}
\newcommand{\nnbr}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

\newcommand{\rsep}[2]{\left(#1 \middle\vert #2 \right)}
\newcommand{\ssep}[2]{\left[#1 \middle\vert #2 \right]}
\newcommand{\csep}[2]{\left\{#1 \middle\vert #2 \right\}}
\newcommand{\asep}[2]{\langle#1 \middle\vert #2 \rangle}
\newcommand{\rsepp}[2]{\left(#1 ~\middle\vert~ #2 \right)}
\newcommand{\ssepp}[2]{\left[#1 ~\middle\vert~ #2 \right]}
\newcommand{\csepp}[2]{\left\{#1 ~\middle\vert~ #2 \right\}}
\newcommand{\asepp}[2]{\langle#1 ~\middle\vert~ #2 \rangle}

\newcommand{\apar}[1]{\langle #1 \rangle}
\newcommand{\cpar}[1]{\{#1\}}
\newcommand{\bpar}[1]{\Big( #1 \Big)}
\newcommand{\Bpar}[1]{\Bigg( #1 \Bigg)}
\newcommand{\bspar}[1]{\Big[ #1 \Big]}
\newcommand{\Bspar}[1]{\Bigg[ #1 \Bigg]}
\newcommand{\bcpar}[1]{\Big\{ #1 \Big\}}
\newcommand{\Bcpar}[1]{\Bigg\{ #1 \Bigg\}}

\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\inpr}[2]{\langle #1, #2 \rangle}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\sembrack}[1]{[\![#1]\!]}

\newcommand{\bmat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\mat}[1]{\begin{pmatrix} #1 \end{pmatrix}}

%%%%%%%%%%%%%%% Python %%%%%%%%%%%%%%%
\definecolor{commentcolor}{RGB}{110,154,155}   % define comment color
\newcommand{\PyComment}[1]{\ttfamily\textcolor{commentcolor}{\# #1}}  % add a "#" before the input text "#1"
\newcommand{\PyCode}[1]{\ttfamily\textcolor{black}{#1}} % \ttfamily is the code font


%%%%%%%%%%%%%%% Miscellaneous %%%%%%%%%%%%%%%
\newcommand{\bs}[1]{\boldsymbol{#1}}
\renewcommand{\b}{\textbf}
\renewcommand{\t}[1]{\text{#1}}
% starred section table of contents
\newcommand{\sectiontoc}[1]{
\section*{#1}
\addcontentsline{toc}{section}{\protect\numberline{}#1}%
}


% Local
% \newcommand{\yd}[1]{\blue{[YD: #1]}}
\newcommand{\needref}{\textcolor{red}{\textbf{@@ref}}}
\newcommand{\todo}[1]{\orange{\b{TODO}: #1}}
\newcommand{\revise}[2]{\orange{\sout{#1} $\to$ #2}}
\newcommand{\add}[1]{\orange{#1}}
\newcommand{\htextwidth}{\noindent\rule{\textwidth}{1pt}}
\newcommand{\vari}{\mathbf{Var}}
\newcommand{\bias}{\mathbf{Bias}}
\newcommand{\stief}{\mathrm{Stiefel}}








